Incremental Learning of 3D-DCT Compact Representations for Robust Visual Tracking

Visual tracking usually requires an object appearance model that is robust to changing illumination, pose and other factors encountered in video. In this paper, we construct an appearance model using the 3D discrete cosine transform (3D-DCT). The 3D-DCT is based on a set of cosine basis functions, which are determined by the dimensions of the 3D signal and thus independent of the input video data. In addition, the 3D-DCT can generate a compact energy spectrum whose high-frequency coefficients are sparse if the appearance samples are similar. By discarding these high-frequency coefficients, we simultaneously obtain a compact 3D-DCT based object representation and a signal reconstruction-based similarity measure (reflecting the information loss from signal reconstruction). To efficiently update the object representation, we propose an incremental 3D-DCT algorithm, which decomposes the 3D-DCT into successive operations of the 2D discrete cosine transform (2D-DCT) and 1D discrete cosine transform (1D-DCT) on the input video data.

==> macros.tex <==


\newcommand{\st}{{\rm s.t.}\xspace}
\newcommand{\trace}{{\bf Tr}}

\def\argmax{\operatorname*{argmax\,}}

%
% Comments
% I use this command to let me make multi-line comments in my latex source:
%
\newcommand{\comment}[1]{}

\def\psd{\succcurlyeq}
\def\nsd{\preccurlyeq}
\def\pd{ \succ }
\def\nd{ \prec }

\def\T{{\!\top}}
\def\transpose{{\!\top}}

\def\Real{\mathbb{R}}

\newcommand{\fnorm}[2][2]{\ensuremath{ \left\| #2 \right\|_{ \mathrm{#1} } } }

\def\x{{\boldsymbol x}}
\def\w{{\boldsymbol w}}



%\theoremstyle{plain}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]

\def\multiboost{{\sc MultiBoost}\xspace}
\def\yi{{  y_i  }}
\newcommand{\mbh}{ {\sc Multi\-Boost}-\-hinge\xspace}
\newcommand{\mbe}{ {\sc Multi\-Boost}-\-exp\xspace}



% EoF


